UniDoorManip: Learning Universal Door Manipulation Policy Over Large-scale and Diverse Door Manipulation Environments

Learning a universal manipulation policy encompassing doors with diverse categories, geometries and mechanisms, is crucial for future embodied agents to effectively work in complex and broad real-world scenarios. Due to the limited datasets and unrealistic simulation environments, previous works fail to achieve good performance across various doors. In this work, we build a novel door manipulation environment reflecting different realistic door manipulation mechanisms, and further equip this environment with a large-scale door dataset covering 6 door categories with hundreds of door bodies and handles, making up thousands of different door instances. Additionally, to better emulate real-world scenarios, we introduce a mobile robot as the agent and use the partial and occluded point cloud as the observation, which are not considered in previous works while possessing significance for real-world implementations. To learn a universal policy over diverse doors, we propose a novel framework disentangling the whole manipulation process into three stages, and integrating them by training in the reversed order of inference. Extensive experiments validate the effectiveness of our designs and demonstrate our framework's strong performance. Code, data and videos are avaible on https://unidoormanip.github.io/.

==> fig/ablation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/ablation.png}
    \caption{Enter Caption}
    \label{fig:ablation}
\vspace{-4mm}
\end{figure}

==> fig/ablation_line.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={Door Joint Angle $\theta_{d}$(°)},
        ylabel={Success Rate},
        xmin = 0, xmax = 60,
        ymin = 0, ymax = 1,
        axis lines = left,
        ymajorgrids=true,
        tick align=outside,
        legend style={at={(0.31,0.44)},anchor=north}
    ]
        %
        \addplot[
            smooth,
            color = Cerulean,
            mark = x,
            line width = 2pt,
            mark size = 3pt
        ]
        coordinates{
            (5,0.910372222)(15,0.905927778)(30,0.89815)(45,0.842588889)(60,0.696666667)
        };
        \addlegendentry{Ours};
        %
        \addplot[
            smooth,
            color = Goldenrod,
            mark = triangle,
            line width = 2pt,
            mark size = 3pt
        ]
        coordinates{
            (5,0.861455556)(15,0.852566667)(30,0.661169444)(45,0.5353)(60,0.396838889)
        };
        \addlegendentry{Ours w/o mobile};
        %
        \addplot[
            smooth,
            color = Gray,
            mark = diamond,
            line width = 2pt,
            mark size = 3pt
        ]
        coordinates{
            (5,0.809052778)(15,0.794619444)(30,0.776841667)(45,0.416241667)(60,0.243161111)
        };
        \addlegendentry{Ours w/o state};
        %
        \addplot[
            smooth,
            color = orange,
            mark = o,
            line width = 2pt,
            mark size = 3pt
        ]
        coordinates{
            (5,0.643236111)(15,0.627766667)(30,0.592113889)(45,0.506536111)(60,0.387502778)
        };
        \addlegendentry{Ours w/o condition};
        \addplot[
            smooth,
            color = Turquoise,
            mark = pentagon,
            line width = 2pt,
            mark size = 3pt
        ]
        coordinates{
            (5,0.598963889)(15,0.586827778)(30,0.562383333)(45,0.294869444)(60,0.136836111)
        };
        \addlegendentry{Ours w/o disentangle};
    \end{axis}
\end{tikzpicture}

==> tabs/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tb]
\begin{center}
\small
\setlength{\tabcolsep}{2mm}{
\begin{tabular}{c|ccccc|ccccc}

\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Pull Door}} & \multicolumn{5}{c}{\textbf{Push Door}} \\

 & \textbf{Avg.} 
 & \includegraphics[width=0.025\linewidth]{tabs/icons/door.png}
 & \includegraphics[width=0.025\linewidth]{tabs/icons/window.png} 
 & \includegraphics[width=0.05\linewidth]{tabs/icons/car1.jpg} 
 & \includegraphics[width=0.025\linewidth]{tabs/icons/safe.png} 
 & \textbf{Avg.} 
 & \includegraphics[width=0.025\linewidth]{tabs/icons/door.png}
 & \includegraphics[width=0.025\linewidth]{tabs/icons/window.png} 
 & \includegraphics[width=0.05\linewidth]{tabs/icons/car1.jpg} 
 & \includegraphics[width=0.025\linewidth]{tabs/icons/safe.png} \\
\hline 
 GAPartNet &  &   &   &   &   &   &    &   &   &   \\
 DoorGym~\cite{urakami2019doorgym} &  &   &   &   &   &   &    &   &   &   \\
 PartManip~\cite{geng2023partmanip} &  &   &   &   &   &   &    &   &   &  \\
 VAT-MART~\cite{wu2022vatmart} &  &   &   &   &   &   &    &   &   &   \\
 UMPNet~\cite{xu2022umpnet} &  &   &   &   &   &   &    &   &   &   \\
 FlowBot3d~\cite{eisner2022flowbot3d} &  &   &   &   &   &   &    &   &   &   \\
 \textbf{Ours} &  &   &   &   &   &   &    &   &   &   \\
\hline
\end{tabular}
}

\caption{
   % \textbf{Statistic comparisons} between previous dataset and ours. \textbf{com.} indicates composition of bodies and handles.
   }
\label{tab:task}
\end{center}
\end{table*}

==> tabs/door_cfg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[tb]
\begin{center}
   \caption{
   List of randomized parameters in the door environment
   }
 \small

\begin{tabular}{@{}llll@{}}
\toprule
\multicolumn{2}{c}{\textbf{random parameters}} & \multicolumn{1}{c}{\textbf{Scaling Factor Range}} & \textbf{Unit} \\ \midrule
\multicolumn{4}{c}{\textbf{Door physical parameters}}                                                              \\ \midrule
Wall property              & wall location     & y-axis Uniform {[}-200, 200{]}                    & mm            \\
Door Frame Joint Property  & door frame damper & Uniform {[}0.1, 0.2{]}                            & -             \\
                           & door spring       & Uniform{[}0.1, 0.2{]}                             & -             \\
                           &                   &                                                   &               \\
                           &                   &                                                   &               \\ \bottomrule
    \end{tabular}
    \label{tab:doorcfg}
\end{center}
\end{table*}
